Anonymous Card Shuffling and its Applications to Parallel Mixnets

We study the question of how to shuffle $n$ cards when faced with an opponent who knows the initial position of all the cards {\em and} can track every card when permuted, {\em except} when one takes $K< n$ cards at a time and shuffles them in a private buffer "behind your back," which we call {\em buffer shuffling}. The problem arises naturally in the context of parallel mixnet servers as well as other security applications. Our analysis is based on related analyses of load-balancing processes. We include extensions to variations that involve corrupted servers and adversarially injected messages, which correspond to an opponent who can peek at some shuffles in the buffer and who can mark some number of the cards. In addition, our analysis makes novel use of a sum-of-squares metric for anonymity, which leads to improved performance bounds for parallel mixnets and can also be used to bound well-known existing anonymity measures.

==> shuffle.tex <==
\section{An Analysis of Shuffling with a Stash}
Let the cards be given an arbitrary labeling.  Our $K$-card algorithm repeats the following steps:
\begin{enumerate}
\item Shuffle the cards, placing them according to a uniform permutation.
\item Under this new ordering, divide the cards up into consecutive groups of $K$ cards.
\item  For each group of $K$ cards, reset their identifiers randomly, hidden from the
adversary.  
\end{enumerate}
We refer to each repetition as a round.

Let $w_i(t)$ be the probability that the $i$th card after $t$ rounds is the first card from time 0
from the point of view of the adversary.  We drop the dependence on $t$ where the meaning is clear.
Initially $w_1 = 1$, and $w_2 \ldots w_n$ are all 0.
Let $\Phi(t)$ be a potential function $\Phi(t) = (\sum w_i(t)^2) - \frac{1}{n}$,
corresponding to the sum-of-squares metric, $\Phi_t$,
and let $\Delta \Phi(t) = \Phi(t) - \Phi(t+1)$.  
Again, we drop the explicit dependence on $t$ where suitable.

When a group of $K$ cards is shuffled, the change in potential is:

\begin{itemize}
\item For 2 cards with weights $w_i$ and $w_j$:
\begin{eqnarray*}
\Delta \Phi & = & D_{ij} \\
            & = & w_i^2 + w_j^2 - 2((w_i+w_j)/2)^2 \\
            & = & (w_i - w_j)^2 /2.
\end{eqnarray*}
\item For 3 cards with weights $w_i$, $w_j$, and $w_k$:
\begin{eqnarray*}
\Delta \Phi & = & D_{ijk} \\
            & = & w_i^2 + w_j^2 + w_k^2 - 3((w_i+w_j+w_k)/3)^2 \\
            & = & (w_i - w_j)^2/3 + (w_j - w_k)^2 /3 + (w_k - w_i)^2 /3 .
\end{eqnarray*}
\item For $K$ cards with weights $w_{i1}$, $w_{i2}$, and $w_{iK}$:
\begin{eqnarray*}
\Delta \Phi & = & \sum_{k = 1}^K w_{ik}^2 - K \left ( \frac{\sum_{k = 1}^K w_{ik}}{K} \right)^2 \\
            & = & \frac{1}{K}\sum_{1 \leq j < k \leq K}^K \left (w_{ij}-w_{ik}\right)^2.
\end{eqnarray*}
\end{itemize}

\begin{eqnarray*}
\E[\Delta \Phi] & = & \frac{1}{K} \sum_{1 \leq i < j \leq n} \Pr \left( (i,j) \mbox{ are in the same set of } K \mbox{ cards} \right) (w_i - w_j)^2 \\
                & = & \frac{K-1}{K(n-1)} \sum_{i < j} (w_i-w_j)^2 \\
                & = & \frac{K-1}{K(n-1)} \sum_{i < j} (w_i-w_j)^2 \\
                & = & \frac{K-1}{2K(n-1)} \sum_{1 \leq i,j \leq n} (w_i-w_j)^2.
\end{eqnarray*}

Also,
\begin{eqnarray*}
\E[\Delta \Phi/\Phi] & = & \frac{K-1}{2K(n-1)} 
\frac{\sum_{i,j} \left( \left( w_i-1/n\right)-\left(w_j-1/n\right) \right)^2}{\sum_k \left(w_k - 1/n \right)^2}.
\end{eqnarray*}
Let $x_i = w_i - 1/n$ to get
\begin{eqnarray*}
\E[\Delta \Phi/\Phi] & = & \frac{K-1}{2K(n-1)} \frac {\sum_{i,j} (x_i- x_j)^2}  {\sum_k x_k^2}.
\end{eqnarray*}
Interestingly, when $K=n$, we should have mixing in one step, so in this case
$\E[\Delta \Phi/\Phi]$ should be 1.  Notice if that is the case, then perhaps surprisingly the above expression
is independent of the actual $x_i$ values, and then we have immediately:
\begin{eqnarray*}
\E[\Delta \Phi/\Phi] & = & \frac{n(K-1)}{K(n-1)}.
\end{eqnarray*}
We can in fact confirm this easily.  Since $\sum_k x_k = 0$, we have 
$$\sum_{i,j} (x_i- x_j)^2 = \sum_{i,j} (x_i- x_j)^2 + 2 \left(\sum_k x_k\right)^2 = 2n \sum_k x_k^2,$$
and cancellation gives the desired result.  

This gives us fast convergence to the uniform distribution.  
Let $\gamma = \frac{n(K-1)}{K(n-1)}$, and note $\gamma < 1$.  
In particular, 
$$1 -\gamma = \frac{n-K}{K(n-1)} < \frac{1}{K}.$$
Also note $\Phi(0) < 1$.  
We have 
$\E[\Phi(t+1)] = (1-\gamma) \Phi(t)$, and a simple induction yields
$\E[\Phi(t)] = (1-\gamma)^t \Phi(0) \leq K^{-t}$.  

\subsection{Extensions to mixnets with corrupted servers}

*** We need to explain the setting;  parallel servers, some of which are corrupted, which corresponds
to our shuffle scenario.  

For corrupted servers, Bob will know the permutation for the cards
assigned to that server.  In terms of the analysis, we can treat the
permutation as the identity operation, since Bob can simply undo that
permutation.  Let us suppose that there are $n/K$ servers, so that each obtains $K$
cards in each round, and that $m \leq n/K$ servers are uncorrupted.  Following our previous analysis,
we find

\begin{eqnarray*}
\E[\Delta \Phi] & = & \frac{1}{K} \sum_{1 \leq i < j \leq n} \Pr \left( (i,j) \mbox{ are in the same set of } K \mbox{ cards at an uncorrupted server} \right) (w_i - w_j)^2 \\
                & = & \frac{(K-1)}{K(n-1)} \frac{m}{n/K}\sum_{i < j} (w_i-w_j)^2 \\
                & = & \frac{m(K-1)}{n(n-1)} \sum_{i < j} (w_i-w_j)^2 \\
                & = & \frac{K-1}{2n(n-1)} \sum_{1 \leq i,j \leq n} (w_i-w_j)^2.
\end{eqnarray*}

Again, based on our previous analysis, we have
\begin{eqnarray*}
\E[\Delta \Phi/\Phi] & = & \frac{m(K-1)}{n-1}.
\end{eqnarray*}
Now let $\gamma' = \frac{m(K-1)}{(n-1)}$;
if, for example, $m = \epsilon \frac{n-1}{K-1}$ then 
$1- \gamma' = 1-\epsilon$.  
In that case we find 
$\E[\Phi(t)] = (1-\epsilon)^t$.  


